Seeing What a GAN Cannot Generate

Despite the success of Generative Adversarial Networks (GANs), mode collapse remains a serious issue during GAN training. To date, little work has focused on understanding and quantifying which modes have been dropped by a model. In this work, we visualize mode collapse at both the distribution level and the instance level. First, we deploy a semantic segmentation network to compare the distribution of segmented objects in the generated images with the target distribution in the training set. Differences in statistics reveal object classes that are omitted by a GAN. Second, given the identified omitted object classes, we visualize the GAN's omissions directly. In particular, we compare specific differences between individual photos and their approximate inversions by a GAN. To this end, we relax the problem of inversion and solve the tractable problem of inverting a GAN layer instead of the entire generator. Finally, we use this framework to analyze several recent GANs trained on multiple datasets and identify their typical failure cases.

==> figText/fsdtable.tex <==
\begin{table}
   \caption{Comparing \fssshort with FID.} 
   \label{tab:fsd}
   \small % text size of table content
   \centering % center the table
   \begin{tabular}{lccr} % alignment of each column data
   \toprule[\heavyrulewidth]\toprule[\heavyrulewidth]
   \textbf{Model} & \textbf{FID} & \textbf{\fssshort}  \\ 
   \midrule
   ProGAN churches (\citet{karras2018progressive}, \reffig{teaser}) & 15.9 & 15.1 \\ \hline
   WGAN-GP bedrooms (\citet{gulrajani2017improved}, \reffig{models} top) & 61.3 & 428.4 \\
   ProGAN bedrooms (\citet{karras2018progressive}, \reffig{bedroom}) & 16.7  & 85.2 \\
   StyleGAN bedrooms (\citet{karras2019style}, \reffig{models} bottom) & 11.1 & 22.6 \\
   \bottomrule[\heavyrulewidth] 
   \end{tabular}
   \vspace{-0.1in}
\end{table}

==> figText/models.tex <==
\begin{figure*}
\centering
\includegraphics[width=\textwidth]{fig/model-analysis-crop.pdf}
\vspace{-0.1in}
\caption{Comparing different GAN models.  Both models are trained to mimic LSUN-bedrooms.  The \gissfull histograms on the left reveal that WGAN-GP (top) deviates from the true distribution much more than StyleGAN (bottom), identifying segmentation classes that are generated too little and others that are generated too much.  On the right, we show generated images that the segmentation network has identified as containing many pixels of sky and exterior building pixels. Because each component of has an interpretable label, we can directly visualize and understand the failures.}
\lblfig{models}
\vspace{-0.15in}
\end{figure*}

==> figText/residual-scatter.tex <==
\begin{figure*}
\centering
\includegraphics[width=0.75\textwidth]{fig/residual-scatter-crop.pdf}
\vspace{-0.1in}
\caption{Comparison of choice of optimization parameters when inverting an interior representation of a large generator.  Each point represents an algorithm that optimizes over a subset of $\{\delta_i\}$.  The vertical axis shows reconstruction error for pixels, and the horizontal axis shows reconstruction error for the \texttt{layer4} latent representation $\rvr_4$.  The best algorithms are at the lower-left, and the worst are in the upper-right.  Note that the straightforward approaches of optimizing over just $\rvz$ or $\rvr_4$ directly lie in the upper-right, and are dominated by residual approaches.}
\lblfig{residual-scatter}
\vspace{-0.1in}
\end{figure*}
